$\omega$Test: WebView-Oriented Testing for Android Applications

WebView is a UI widget that helps integrate web applications into the native context of Android apps. It provides powerful mechanisms for bi-directional interactions between the native-end (Java) and the web-end (JavaScript) of an Android app. However, these interaction mechanisms are complicated and have induced various types of bugs. To mitigate the problem, various techniques have been proposed to detect WebView-induced bugs via dynamic analysis, which heavily relies on executing tests to explore WebView behaviors. Unfortunately, these techniques either require manual effort or adopt random test generation approaches, which are not able to effectively explore diverse WebView behaviors. In this paper, we study the problem of test generation for WebViews in Android apps. Effective test generation for WebViews requires identifying the essential program properties to be covered by the generated tests. To this end, we propose WebView-specific properties to characterize WebView behaviors, and devise a cross-language dynamic analysis method to identify these properties. We develop $\omega$Test, a test generation technique that searches for event sequences covering the identified WebView-specific properties. An evaluation on 74 real-world open-/closed-source Android apps shows that $\omega$Test can cover diverse WebView behaviors and detect WebView-induced bugs effectively. $\omega$Test detected 36 previously-unknown bugs. From the 22 bugs that we have reported to the app developers, 13 bugs were confirmed, 9 of which were fixed.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/coverage.tex <==
\section{Property}\label{property}
This section presents our proposed coverage criteria for measuring the adequacy of test cases exploring WebViews in Android applications. The proposed criteria are designed based on the access of WebView APIs and the variables propagated from/to these APIs. Therefore, in this section, we will present the variable propagation rules before presenting the proposed criteria.

\subsection{Propagation Rules}
The propagation rules designed by us are illustrated in Table~\ref{table:propagation}. The objective of these rules is to find out WebView-related variables in an Android app. We use a tag function $\omega(x)$ that outputs 0 or 1  to indicate if variable $x$ has relationships with WebViews or not. $\omega(x) = 1$ means $x$ has relationships with WebViews and $\omega(x) = 0$ means $x$ does NOT have relationships with WebViews. The logic to initialize tags is presented in the \emph{Tag Initialization} part of Table~\ref{table:propagation}, while the logic to propagate these tags is presented in the \emph{Forward/Backward Propagation} parts of Table~\ref{table:propagation}.

\textbf{Tag Initialization:} We initialize variable tags according to WebView semantics. (1) The tags of parameters of WebView callback methods are initialized to be 1. The reason is that these parameters pass the information of events occurring at the web-end of an Android app to its native-end. For example, a callback method \texttt{shouldOverrideUrlLoading(WebView view, WebResourceRequest request)} is triggered when a URL is about to be loaded by a WebView. One of its parameters \texttt{request} carries the details of the URL request that happened at the web end. (2) The tags of the parameters and the tags of the return variable of bridge methods~\cite{lee2016hybridroid} declared in Java code are initialized to be 1. The reason is that bridge methods are Java methods that are available to the JavaScript code on a web page. The parameter values of bridge methods are passed from JavaScript code, and the computing result is also returned back to JavaScript code. (3) The tags of the parameters of bridge method calls and the tags of the variables that take the return value in JavaScript code are initialized to be 1. The reason is that these parameters are passed to Java code, and the result of method calls is also returned from Java code. (4) Several WebView APIs (e.g., \texttt{loadUrl()}) are responsible for injecting and executing JavaScript code into the pages loaded by WebViews. The tags of the constant variables in the injected JavaScript code are initialized to be 1. The reason is that the value of these constant variables is given by Java code and these variables will be further processed by JavaScript code. For example, the 2 parameters of \texttt{handleMessage()} at line 11 of Figure~\ref{fig:trace} are treated as constant variables when analyzing \texttt{jsString} at line 12 because their values are given by \texttt{msgName} and \texttt{msgPointer}. 

\textbf{Forward/Backward Propagation:} The initialized tags will be propagated according to the forward/backward propagation rules specified in Table~\ref{table:propagation}. We abstract 3 types of instructions (i.e., unary operation, binary operation, and library method call) to propagate tags based on a data-flow logic. We do not include a control-flow logic as it could introduce too much noise (e.g., it is hard to say a variable is WebView-related if it is control dependent on a WebView-related variable). Tags are propagated forward to find out the variables affected by WebView-related variables. For example, the tag of \texttt{payload} at line 15 of Figure~\ref{fig:trace} will be propagated from the tag of the parameter of the library method call \texttt{JSON.parse()} (the tag value should be 1 because the parameter value is returned from a bridge method call \texttt{marshaller.putPayload()}). Tags are also propagated backward from the web-native interaction points of WebView to find out the variables that affect the interactions. For example, the tag values of \texttt{msgName} and \texttt{msgPointer} at line 11 of Figure~\ref{fig:trace} will be propagated backward from the tag value of \texttt{jsString} at line 12.



\begin{table*}
	%\renewcommand{\arraystretch}{1.0}
	%\small
	\begin{center}
		\caption{Propagation Rules}
		\begin{tabular}{| c | c | c | c |}
			\ChangeRT{1pt}
			\textbf{} & \textbf{Operation Semantics} & \textbf{Propagation rules} & \textbf{Description}\\
			\hline
			\multirow{3}{*}{\makecell{Forward Propagation}} & $x = [op]\;y$ & $\omega(y) \rightarrow \omega(x)$ & \\
			\cline{2-4}
			& $x = y\;op\;z$ & $\omega(y) | \omega(z) \rightarrow \omega(x)$ & \\
			\cline{2-4}
			& $x = libcall(y_1, y_2, ..., y_n)$ & $\omega(y_1) | \omega(y_2) | ... | \omega(y_n) \rightarrow \omega(x)$ & \\
			\hline
			\multirow{3}{*}{\makecell{Backward Propagation}} & $x = [op]\;y$ & $\omega(x) \rightarrow \omega(y)$ & \\
			\cline{2-4}
			& $x = y\;op\;z$ & \makecell{$\omega(x) \rightarrow \omega(y)$ \\ $\omega(x) \rightarrow \omega(z)$} & \\
			\cline{2-4}
			& $x = libcall(y_1, y_2, ..., y_n)$ & \makecell{$\omega(x) \rightarrow \omega(y_1)$ \\ $\omega(x) \rightarrow \omega(y_2)$ \\ $...$ \\ $\omega(x) \rightarrow \omega(y_n)$} & \\
			\hline
			\multirow{4}{*}{\makecell{Tag Initialization}} & $callback(y_1, y_2, ..., y_n)$ & $\omega(y_1)=1, \omega(y_2)=1, ..., \omega(y_n)=1$ & \\
			\cline{2-4}
			& \makecell{$bridgeMtd(y_1, y_2, ..., y_n)$ \\ $\{... return\;r;\}$} & $\omega(y_1)=1, \omega(y_2)=1, ..., \omega(y_n)=1, \omega(r) = 1$ & \\
			\cline{2-4}
			& $x = bridgeCall(y_1, y_2, ..., y_n)$ &$\omega(y_1)=1, \omega(y_2)=1, ..., \omega(y_n)=1, \omega(x) = 1$ & \\
			\cline{2-4}  
			& $execJS(jsCode)$& $\{\omega(x)=1 | x\in jsCode \wedge isConst(x) = true\}$ & \\
			\ChangeRT{1pt}
		\end{tabular}
		\label{table:propagation}
	\end{center}
\end{table*}


\subsection{Criteria}
Having found out the WebView-related variables from both the native end and the web end of an Android app, the new criteria designed by us is based on the access of these variables. 
\begin{definition}[\wCov]
	A set of test cases satisfies the coverage criteria iff all feasible values of all variables x such that $\omega(x)=1$ are covered.
\end{definition}

The proposed criteria treat every WebView-related variable with the value taken by it as one property to be covered by a test case. For example, variable \texttt{window.apiLevel} at line 24 of Figure~\ref{fig:trace} is treated as a WebView-related variable according to the propagation rules specified in Table~\ref{table:propagation}. Two test cases cover different properties if the value of \texttt{window.apiLevel} is 19 in one test case and the value of \texttt{window.apiLevel} is 20 in another test case.

%\begin{itemize}[label=\textbullet, leftmargin=*, itemsep=2pt]
%	\item \textbf{Criterion 1: variable-access coverage (C1)} \emph{A set of test cases satisfies the C1 criterion iff for all WebView-related variables \wvarws$\in$ V, there is at least one test case whose execution accesses \wvar.} 
%\end{itemize}
%The property to be covered under this criterion is a WebView-related variable \wvar. A test case covers different properties if it accesses different variables \jiajun{I should define what are different \wvar s. Actually I treat variables used in different program locations as different variables even they are the uses of the same def}.


%\begin{itemize}[label=\textbullet, leftmargin=*, itemsep=2pt]
%	\item \textbf{Criterion 2(b): variable-access-order coverage (C3)}
%\end{itemize}
%We motivate this coverage criteria because some WebView-induced bugs can be triggered only under specific variable access order.

